Wave dispersion in pulsar plasma: 1. Plasma rest frame

Wave dispersion in a pulsar plasma (a 1D, strongly magnetized, pair plasma streaming highly relativistically with a large spread in Lorentz factors in its rest frame) is discussed, motivated by interest in beam-driven wave turbulence and the pulsar radio emission mechanism. In the rest frame of the pulsar plasma there are three wave modes in the low-frequency, non-gyrotropic approximation. For parallel propagation these are referred to as the X, A and L modes, with the X and A modes having dispersion relation $z=z_A\approx1-1/2\beta_A^2$, where $z=\omega/k_\parallel c$ is the phase speed and $\beta_Ac$ is the Alfven speed. The L mode dispersion relation is determined by a relativistic plasma dispersion function, $z^2W(z)$, which is negative for $ z < z_0 $ and has a sharp maximum at $z=z_m$, with $1-z_m<1-z_0\ll1$. We give numerical estimates for the maximum of $z^2W(z)$ and for $z_m$ and $z_0$ for a 1D Juttner distribution. The L and A modes reconnect, for $z_A>z_0$, to form the O and Alfven modes for oblique propagation ($\theta\neq0$). For $z_A<z_0$ the Alfven and O~mode curves reconnect forming a new mode that exists only for $\tan^2\theta>z_0^2-z_A^2$. The L mode is the nearest counterpart to Langmuir waves in a nonrelativistic plasma, but we argue that there are no `Langmuir-like' waves in pulsar plasma, identifying three features of the L~mode (dispersion relation, ratio of electric to total energy and group speed) that are not Langmuir-like. A beam-driven instability requires a beam speed equal to the phase speed of the wave. This resonance condition can be satisfied for the O mode, but only for an implausibly energetic beam and only for a tiny range of angles for the O~mode around $\theta\approx0$. The resonance is also possible for the Alfven mode but only near a turnover frequency that has no counterpart for Alfven waves in a nonrelativistic plasma.

==> fig1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $ z $}%
\psfrag{013}[bc][bc]{\matlabtextA $ z^2W(z) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{002}[ct][ct]{\matlabtextB $1$}%
\psfrag{003}[ct][ct]{\matlabtextB $1.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $-3$}%
\psfrag{005}[rc][rc]{\matlabtextB $-2$}%
\psfrag{006}[rc][rc]{\matlabtextB $-1$}%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $1$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $3$}%
\psfrag{011}[rc][rc]{\matlabtextB $4$}%
%
%% </ytick>

==> fig10a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{009}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig10b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{009}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig11.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{015}[bc][bc]{\matlabtextA $ \rho^2/R_L(z) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.01$}%
\psfrag{001}[ct][ct]{\matlabtextB ${}$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB ${}$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.01$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB ${}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10$}%
\psfrag{008}[rc][rc]{\matlabtextB ${}$}%
\psfrag{009}[rc][rc]{\matlabtextB $20$}%
\psfrag{010}[rc][rc]{\matlabtextB ${}$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB ${}$}%
\psfrag{013}[rc][rc]{\matlabtextB $40$}%
%
%% </ytick>

==> fig12.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{017}[bc][bc]{\matlabtextA $ \rho^2/[1-\beta_{\rm g}(z)] $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.01$}%
\psfrag{001}[ct][ct]{\matlabtextB ${}$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB ${}$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.01$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB ${}$}%
\psfrag{007}[rc][rc]{\matlabtextB $4$}%
\psfrag{008}[rc][rc]{\matlabtextB ${}$}%
\psfrag{009}[rc][rc]{\matlabtextB $8$}%
\psfrag{010}[rc][rc]{\matlabtextB ${}$}%
\psfrag{011}[rc][rc]{\matlabtextB $12$}%
\psfrag{012}[rc][rc]{\matlabtextB ${}$}%
\psfrag{013}[rc][rc]{\matlabtextB $16$}%
\psfrag{014}[rc][rc]{\matlabtextB ${}$}%
\psfrag{015}[rc][rc]{\matlabtextB $20$}%
%
%% </ytick>

==> fig2a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{017}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{018}[bc][bc]{\matlabtextA $ \rho z^2W(z) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextB $0$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $1.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB ${}$}%
\psfrag{006}[rc][rc]{\matlabtextB $-2$}%
\psfrag{007}[rc][rc]{\matlabtextB ${}$}%
\psfrag{008}[rc][rc]{\matlabtextB $-1$}%
\psfrag{009}[rc][rc]{\matlabtextB ${}$}%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB ${}$}%
\psfrag{012}[rc][rc]{\matlabtextB $1$}%
\psfrag{013}[rc][rc]{\matlabtextB ${}$}%
\psfrag{014}[rc][rc]{\matlabtextB $2$}%
\psfrag{015}[rc][rc]{\matlabtextB ${}$}%
\psfrag{016}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> fig2b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{018}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{019}[bc][bc]{\matlabtextA $ \rho z^2W(z) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.1$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.05$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.05$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB ${}$}%
\psfrag{007}[rc][rc]{\matlabtextB $-2$}%
\psfrag{008}[rc][rc]{\matlabtextB ${}$}%
\psfrag{009}[rc][rc]{\matlabtextB $-1$}%
\psfrag{010}[rc][rc]{\matlabtextB ${}$}%
\psfrag{011}[rc][rc]{\matlabtextB $0$}%
\psfrag{012}[rc][rc]{\matlabtextB ${}$}%
\psfrag{013}[rc][rc]{\matlabtextB $1$}%
\psfrag{014}[rc][rc]{\matlabtextB ${}$}%
\psfrag{015}[rc][rc]{\matlabtextB $2$}%
\psfrag{016}[rc][rc]{\matlabtextB ${}$}%
\psfrag{017}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> fig3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextB $ z_{\rm e2}^2 \Im W(z_{\rm e2}) $}%
\psfrag{016}[cl][cl]{\matlabtextB $ z_{\rm e1}^2 \Im W(z_{\rm e1}) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $z_{\rm e2}$}%
\psfrag{002}[ct][ct]{\matlabtextB $z_{\rm min}$}%
\psfrag{003}[ct][ct]{\matlabtextB $z_0$}%
\psfrag{004}[ct][ct]{\matlabtextB $z_{\rm Imin}$}%
\psfrag{005}[ct][ct]{\matlabtextB $z_{\rm e1}$}%
\psfrag{006}[ct][ct]{\matlabtextB $z_{\rm m}$}%
\psfrag{007}[ct][ct]{\matlabtextB $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $z_{\rm Imin}^2 \Im W(z_{\rm Imin})$}%
\psfrag{009}[rc][rc]{\matlabtextB ${}$}%
\psfrag{010}[rc][rc]{\matlabtextB $z_{\rm min}^2 \Re W(z_{\rm min})$}%
\psfrag{011}[rc][rc]{\matlabtextB ${}$}%
\psfrag{012}[rc][rc]{\matlabtextB $0$}%
\psfrag{013}[rc][rc]{\matlabtextB $z_{\rm e1}^2 \Re W(z_{\rm e1})$}%
\psfrag{014}[rc][rc]{\matlabtextB $z_{\rm m}^2 \Re W(z_{\rm m})$}%
%
%% </ytick>

==> fig4a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{007}[tc][tc]{\matlabtextA $ \rho $}%
\psfrag{008}[bc][bc]{\matlabtextA $ \gamma_\phi $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{-2}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{-1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{1}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>

==> fig4b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{007}[tc][tc]{\matlabtextA $ \rho $}%
\psfrag{008}[bc][bc]{\matlabtextA $ z^2 W(z) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{-2}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{-1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{1}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>

==> fig5.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[tl][tl]{\matlabtextA $ \omega = ck_\parallel $}%
\psfrag{021}[tl][tl]{\matlabtextA X}%
\psfrag{022}[tl][tl]{\matlabtextA LO}%
\psfrag{023}[tl][tl]{\matlabtextA $ \theta = 10^{-6} $}%
\psfrag{024}[tl][tl]{\matlabtextA $ \theta = 0 $}%
\psfrag{025}[tl][tl]{\matlabtextA $ \theta = 0.5 $}%
\psfrag{026}[tl][tl]{\matlabtextA Alfv\'{e}n}%
\psfrag{027}[tl][tl]{\matlabtextA $ \theta = 0.25 $}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{028}[tc][tc]{\matlabtextB $ c k_\parallel/\omega_{p} $}%
\psfrag{029}[bc][bc]{\matlabtextB $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $$}%
\psfrag{004}[ct][ct]{\matlabtextC $5$}%
\psfrag{010}[ct][ct]{\matlabtextC $0$}%
\psfrag{011}[ct][ct]{\matlabtextC $$}%
\psfrag{012}[ct][ct]{\matlabtextC $1$}%
\psfrag{013}[ct][ct]{\matlabtextC $$}%
\psfrag{014}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[lc][lc]{\matlabtextC $-5$}%
\psfrag{006}[lc][lc]{\matlabtextC $$}%
\psfrag{007}[lc][lc]{\matlabtextC $0$}%
\psfrag{008}[lc][lc]{\matlabtextC $$}%
\psfrag{009}[lc][lc]{\matlabtextC $5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0$}%
\psfrag{016}[rc][rc]{\matlabtextC $$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
\psfrag{018}[rc][rc]{\matlabtextC $$}%
\psfrag{019}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> fig6.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $ ck_{\parallel}/\omega_{\rm p}$}%
\psfrag{013}[bc][bc]{\matlabtextA $ \omega/\omega_{\rm p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $$}%
\psfrag{001}[ct][ct]{\matlabtextB $1$}%
\psfrag{002}[ct][ct]{\matlabtextB $$}%
\psfrag{003}[ct][ct]{\matlabtextB $2$}%
\psfrag{004}[ct][ct]{\matlabtextB $$}%
\psfrag{005}[ct][ct]{\matlabtextB $3$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> fig7.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextA $ ck_{\parallel}/\omega_{\rm p}$}%
\psfrag{021}[bc][bc]{\matlabtextA $ \omega/\omega_{\rm p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $$}%
\psfrag{001}[ct][ct]{\matlabtextB $$}%
\psfrag{002}[ct][ct]{\matlabtextB $$}%
\psfrag{003}[ct][ct]{\matlabtextB $$}%
\psfrag{004}[ct][ct]{\matlabtextB $1$}%
\psfrag{005}[ct][ct]{\matlabtextB $$}%
\psfrag{006}[ct][ct]{\matlabtextB $$}%
\psfrag{007}[ct][ct]{\matlabtextB $$}%
\psfrag{008}[ct][ct]{\matlabtextB $$}%
\psfrag{009}[ct][ct]{\matlabtextB $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $$}%
\psfrag{011}[rc][rc]{\matlabtextB $$}%
\psfrag{012}[rc][rc]{\matlabtextB $$}%
\psfrag{013}[rc][rc]{\matlabtextB $$}%
\psfrag{014}[rc][rc]{\matlabtextB $1$}%
\psfrag{015}[rc][rc]{\matlabtextB $$}%
\psfrag{016}[rc][rc]{\matlabtextB $$}%
\psfrag{017}[rc][rc]{\matlabtextB $$}%
\psfrag{018}[rc][rc]{\matlabtextB $$}%
\psfrag{019}[rc][rc]{\matlabtextB $2$}%
%
%% </ytick>

==> fig8a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{010}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.8$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.6$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.2$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig8b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{009}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.8$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.6$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.2$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig9a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{007}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{008}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.05$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig9b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{006}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{007}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.05$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>
